ChainStream: An LLM-based Framework for Unified Synthetic Sensing

Many applications demand context sensing to offer personalized and timely services. Yet, developing sensing programs can be challenging for developers and using them is privacy-concerning for end-users. In this paper, we propose to use natural language as the unified interface to process personal data and sense user context, which can effectively ease app development and make the data pipeline more transparent. Our work is inspired by large language models (LLMs) and other generative models, while directly applying them does not solve the problem - letting the model directly process the data cannot handle complex sensing requests and letting the model write the data processing program suffers error-prone code generation. We address the problem with 1) a unified data processing framework that makes context-sensing programs simpler and 2) a feedback-guided query optimizer that makes data query more informative. To evaluate the performance of natural language-based context sensing, we create a benchmark that contains 133 context sensing tasks. Extensive evaluation has shown that our approach is able to automatically solve the context-sensing tasks efficiently and precisely. The code is opensourced at https://github.com/MobileLLM/ChainStream.

==> tex/S3_overview.tex <==
\section{Overview}

\jiacheng{This part is written for old version of the paper, which generator is not included in the framework, so need to discuss whether to keep this part or not.}

To better achieve our objectives, the \sys system consists of three main components: the \sys framework, an \generator and a context sensing Benchmark. The \sys framework is a stream-based framework specifically designed for continuous context sensing tasks. It includes streaming encapsulation and multi-device association for data from various source sensors, a streaming computation graph for executing sensing tasks with multiple agents, and a specially designed streamlined API. The \generator provides a tool to automatically generate \sys agents based on user-provided descriptions of requirements, primarily using a feedback guided in-context learning approach for programming and debugging with an LLM agent. The feedback comes from our specially designed agent simulation environment, the sandbox. The sensing Benchmark includes a set of tasks simulating real-world context sensing scenarios with data, and a set of metrics for evaluating the performance of context sensing agents. 


The components of the system are closely interconnected: the \sys framework provides the APIs used during development and ultimately runs the agents. The core of the Sandbox in the \generator is the framework’s Runtime, which also supplies the generator with the sandbox and numerous evaluation tasks. The primary foundation for the Agent Generator’s ability to complete generation tasks is the concise design of the \sys API and the feedback provided by the sandbox on errors and results. The sensing Benchmark provides a set of tasks and metrics for evaluating the performance of context sensing agents.

Next, we will discuss the main design of the \sys framework in Section 4, introduce the \generator in Section 5, and present the benchmark in Section 6.

==> tex/S8_case_study.tex <==
\section{case study}

show some computation graph for real-world application. like smart office, smart lab...

when chainstream package integate into LangChain and other framework...

==> tex/S9_discuss_and_future_work.tex <==
\section{Discussion and Future work}

shortage:
\begin{itemize}
    \item xxx
\end{itemize}


future work:
\begin{itemize}
    \item make system more stable
    \item make bigger agent store
    \item try more complex tasks
    \item more runtime optimization
\end{itemize}

